Integrating Reason-Based Moral Decision-Making in the Reinforcement Learning Architecture

Reinforcement Learning is a machine learning methodology that has demonstrated strong performance across a variety of tasks. In particular, it plays a central role in the development of artificial autonomous agents. As these agents become increasingly capable, market readiness is rapidly approaching, which means those agents, for example taking the form of humanoid robots or autonomous cars, are poised to transition from laboratory prototypes to autonomous operation in real-world environments. This transition raises concerns leading to specific requirements for these systems - among them, the requirement that they are designed to behave ethically. Crucially, research directed toward building agents that fulfill the requirement to behave ethically - referred to as artificial moral agents(AMAs) - has to address a range of challenges at the intersection of computer science and philosophy. This study explores the development of reason-based artificial moral agents (RBAMAs). RBAMAs are build on an extension of the reinforcement learning architecture to enable moral decision-making based on sound normative reasoning, which is achieved by equipping the agent with the capacity to learn a reason-theory - a theory which enables it to process morally relevant propositions to derive moral obligations - through case-based feedback. They are designed such that they adapt their behavior to ensure conformance to these obligations while they pursue their designated tasks. These features contribute to the moral justifiability of the their actions, their moral robustness, and their moral trustworthiness, which proposes the extended architecture as a concrete and deployable framework for the development of AMAs that fulfills key ethical desiderata. This study presents a first implementation of an RBAMA and demonstrates the potential of RBAMAs in initial experiments.

==> config.tex <==

\title{Integrating Reason-Based Moral Decision-Making in the Reinforcement Learning Architecture}
\setauthor{Lisa Dargasz}
\setcity{Saarbrücken}
\setsubmissiondate{29}{April}{2025}

% Decide whether or not you want the beloved own on the title page.
\setboolean{titlepagelogo}{true}
% Determines the placement of the owl.  Hard to explain, try out both.
\setboolean{logobottom}{true}
% Determines whether or not you are writing a dissertation or a bachelor/master thesis.
% Has an impact on the frontmatter.
\setboolean{dissertation}{false}
% Turn night mode on or off.
\setboolean{nightmode}{false}
% Switch XeLaTeX on or off. Generally, if the xelatex version is running, it simplifies a couple things.  Changes fonts.
% If either of the font sets is fine for you, use xelatex until you encounter a problem.  You'll find more support online for regular latex.
\setboolean{xelatex}{false}
% Allows you to include a statement that the print version and the digital versions are congruent.
% This is required for the print versions at Saarland University.
\setboolean{printversion}{true}
% Shows or hides frames. Useful for finding overfull boxes.
\setboolean{showframes}{false}

% This is the marker that is used in text before cross references.  Empty by default can e.g. be `\MVRightarrow\thinspace ' for an arrow in front of it, such as `-> Definition 5'.
\newcommand*\intextcrossrefmarker{}
%\renewcommand*\intextcrossrefmarker{\MVRightarrow\thinspace}


\ifthenelse{\boolean{dissertation}}{

}{
  \setexaminerone{Prof.~Verena  Wolf}
  \setexaminertwo{Dr.~Kevin Baum}
  \setadvisor{Felix Jahn}
  \setadvisortwo{Dr.~Kevin Baum}
  
  \setsupervisor{Prof.~Verena Wolf}
  \setthesiskind{Master}
  \setuniversity{Saarland University}
  \setdepartment{Department of Computer Science}
}



==> internals.tex <==
\RequirePackage{ifthenx}
\RequirePackage{etoolbox}
\RequirePackage{marginnote}
\RequirePackage{mparhack}
\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}
\RequirePackage[Lenny]{fncychap}
\RequirePackage[headsepline=.6pt,footsepline=false]{scrlayer-scrpage}
\RequirePackage{scrhack} 
\RequirePackage{xcolor} 
\RequirePackage[inline]{enumitem} 
\RequirePackage{amsthm}
\RequirePackage{thmtools}
\RequirePackage{array}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Prepare new commands
\newcommand*{\setauthor}[1]{\newcommand*{\AUTHOR}{#1}}
\newcommand*{\setexaminerone}[1]{\newcommand*{\EXAMINERONE}{#1}}
\newcommand*{\setexaminertwo}[1]{\newcommand*{\EXAMINERTWO}{#1}}
\newcommand*{\setexaminerthree}[1]{\newcommand*{\EXAMINERTHREE}{#1}}
\newcommand*{\setexaminerfour}[1]{\newcommand*{\EXAMINERFOUR}{#1}}
\newcommand*{\setadvisor}[1]{\newcommand*{\ADVISOR}{#1}}
\newcommand*{\setadvisortwo}[1]{\newcommand*{\ADVISORTWO}{#1}}
\newcommand*{\setsupervisor}[1]{\newcommand*{\SUPERVISOR}{#1}}
\newcommand*{\setdean}[1]{\newcommand*{\DEAN}{#1}}
\newcommand*{\setdefensedate}[1]{\newcommand*{\DEFENSEDATE}{#1}}
\newcommand*{\setthesiskind}[1]{\newcommand*{\THESISKIND}{#1}}
\newcommand*{\setuniversity}[1]{\newcommand*{\UNIVERSITY}{#1}}
\newcommand*{\setdepartment}[1]{\newcommand*{\DEPARTMENT}{#1}}
\newcommand*{\setcity}[1]{\newcommand*{\CITY}{#1}}
\newcommand*{\setsubmissiondate}[3]{
  \newcommand*{\SUBMISSIONDAY}{#1}
  \newcommand*{\SUBMISSIONMONTH}{#2}
  \newcommand*{\SUBMISSIONYEAR}{#3}
}

% The following commands allow us to use the usual title command for declaring the title.
% The reason is that several editors set the project's title to the argument of \title.
% We store the usual definition of \title in \constructtitle, use it later and renew \title itself.
\let\constructtitle\title{}
\renewcommand*{\title}[1]{\newcommand*{\TITLE}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Define configurable bool flags

\newboolean{titlepagelogo}
\newboolean{logobottom}
\newboolean{dissertation}
\newboolean{nightmode}
\newboolean{xelatex}
\newboolean{printversion}
\newboolean{showframes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Include bool configurations

\input{config}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Import geometry 

% The first shows the dimensions, makes it easier to detect inconsistencies. Switch to latter before submission.
\ifthenelse{\boolean{showframes}}{
	\usepackage[showframe]{geometry}
}{\usepackage{geometry}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Patches and Hacks 

% Fix misaligned line numbers:
% https://tex.stackexchange.com/questions/476579/how-to-align-line-numbers-horizontally-with-package-algorithm2e
\makeatletter
\patchcmd\algocf@Vline{\vrule}{\vrule \kern-0.4pt}{}{}
\patchcmd\algocf@Vsline{\vrule}{\vrule \kern-0.4pt}{}{}
\makeatother

% Fix for deprecated font command
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathsf}

% Ugly hack to get useful \vdots, taken from http://tex.stackexchange.com/a/112212
\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}\hbox{.}\hbox{.}
  }}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Labels and References

\NewDocumentCommand{\CrefAbbrevNames}{}{%
	\Crefname{definition}{Def.}{Defs.}%
	\Crefname{section}{Sec.}{Secs.}%
	\Crefname{examplex}{Ex.}{Exs.}%
	\Crefname{equation}{Eq.}{Eqs.}%
	\Crefname{proposition}{Prop.}{Props.}%
	\Crefname{lemma}{Lem.}{Lems.}%
	\Crefname{corollary}{Cor.}{Cors.}%
	\Crefname{theorem}{Thm.}{Thms.}%
	\Crefname{remark}{Rem.}{Rems.}%
	\Crefname{figure}{Fig.}{Figs.}%
	\Crefname{table}{Tbl.}{Tbls.}%
	\Crefname{algorithm}{Alg.}{Algs.}%
}

\NewDocumentCommand{\shortCref}{ s m }{{% The nested block here is important.
\CrefAbbrevNames%
\renewcommand{\crefrangeconjunction}{--}%
\renewcommand{\crefpairconjunction}{, }%
%    \renewcommand{\crefmiddleconjunction}{⟨conjunction ⟩} 
\renewcommand{\creflastconjunction}{, }%
\Cref{#2}%
}}
  
\newcommand{\MarginCrossRef}[1]{%
\raggedmarginpar{%
  \scriptsize \MVRightarrow\,\shortCref{#1}, p.~\labelcpageref{#1}}%
}

\newcommand{\CCref}[1]{\intextcrossrefmarker{}\Cref{#1}\MarginCrossRef{#1}}

\NewDocumentCommand{\introterm}{ s o m }{% Print optional 2nd arg if it exists, otherwise 3rd.
  \raggedmarginpar{\scriptsize%
    \IfBooleanTF{#1}{%
	    \IfValueTF{#2}{#2}{#3}%
    }{%
    	\textbf{Def.}~\IfValueTF{#2}{#2}{#3}% Add Def. only if star is not there.
    }%
  }%
  \emph{#3}%
}

\newcommand*\raggedmarginpar[1]{\marginpar[{\raggedleft #1}]{\raggedright #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Theorem Environments

\newcommand*\Vhrulefill[1]{\leavevmode\leaders\hrule height 1ex depth \dimexpr#1-1ex\hfill}
\newcommand*{\defheaderline}{{\color{lightgray}\Vhrulefill{1pt}}\par}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Templates for the Statement and Congruence pages

\newcommand{\STATEMENTPAGE}{
  \vspace*{2cm}

  \noindent\textbf{Eidesstattliche Erkl\"arung}

  \noindent Ich erkl\"are hiermit an Eides Statt, dass ich die vorliegende Arbeit
  selbst\"andig verfasst und keine anderen als die angegebenen Quellen und
  Hilfsmittel verwendet habe.

  \bigskip
  \noindent\textbf{Statement in Lieu of an Oath}

  \noindent I hereby confirm that I have written this thesis on my own and that I
  have not used any other media or materials than the ones referred to in
  this thesis.


  \vspace{5cm}

  \noindent\textbf{Einverst\"andniserkl\"arung}

  \noindent Ich bin damit einverstanden, dass meine (bestandene) Arbeit in beiden
  Versionen in die Bibliothek der Informatik aufgenommen und damit
  ver\"offentlicht wird.

  \bigskip
  \noindent\textbf{Declaration of Consent}

  \noindent I agree to make both versions of my thesis (with a passing grade)
  accessible to the public by having them added to the library of the
  Computer Science Department.

  \vspace*{5cm}
  \noindent\rule{8cm}{.4pt}\\[\medskipamount]
  \CITY, \SUBMISSIONDAY\ \SUBMISSIONMONTH, \SUBMISSIONYEAR{}

  \cleardoublepage{}
}

\newcommand{\CONGRUENCESTATEMENT}{
  \vspace*{2cm}

  \noindent\textbf{Erkl\"arung}

  \noindent Ich erkläre hiermit, dass die vorliegende Arbeit mit der elektronischen Version übereinstimmt.

  \bigskip
  
  \noindent\textbf{Statement}

  \noindent I hereby confirm the congruence of the contents of the printed data and the electronic version of the thesis.

  \vspace*{3cm}
  \noindent\rule{8cm}{.4pt}\\[\medskipamount]
  \CITY, \SUBMISSIONDAY\ \SUBMISSIONMONTH, \SUBMISSIONYEAR{}

  \cleardoublepage{}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Adjust some values and lengths

% Punish widows and orphans because we're awful people:
\widowpenalty10000
\clubpenalty10000

% Enable emergency stretches because we don't mind a few empty points.
\emergencystretch=10pt

% Set the margin par width appropriately
\setlength{\marginparwidth}{2.8cm} 

% Increase distance between array rows
\renewcommand\arraystretch{1.5}
\setlength{\jot}{8pt}

\setdescription{topsep=10pt,itemsep=0pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Font Style

\ifthenelse{\boolean{xelatex}}{
  \usepackage{fontspec}
  % \usepackage{zi4} % Nice monospace font
  \usepackage[scaled=0.84]{beramono}
  \setmainfont[ 
      BoldFont       = texgyrepagella-bold.otf,
      ItalicFont     = texgyrepagella-italic.otf,
      BoldItalicFont = texgyrepagella-bolditalic.otf ]
    {texgyrepagella-regular.otf}
  \usepackage{unicode-math}
  \setmathfont{Asana-Math.otf}
}{
  \usepackage[utf8]{inputenc}
  \usepackage[T1]{fontenc}
  \usepackage[scaled=0.88]{beraserif}
  \usepackage[scaled=0.85]{berasans}
  \usepackage[scaled=0.84]{beramono}
  \usepackage{newpxtext}
  \usepackage[T1,small,euler-digits]{eulervm} % Euler Math Font
  \linespread{1.05}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Headers and Footers

% Change \leftmark for chapters to be of form e.g. `1. Introduction`.
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.~#1}{}}
% Change \rightmark for sections to be of form e.g. `1.2. Related Work`.
\renewcommand{\sectionmark}[1]{\markright{\thesection.~#1}}

% Set chapter numbers to Helvetica.
\ChNumVar{\fontsize{60}{62}\usefont{OT1}{phv}{m}{n}\selectfont}
% \ChNumVar{\fontsize{60}{62}\normalfont}

\ifthenelse{\boolean{xelatex}}{
  \ChTitleVar{\fontsize{30}{33}\bfseries\sffamily}
}{
  \ChTitleVar{\fontsize{30}{33}\bfseries\sffamily\selectfont}
}

% Allows you to move the footer and page number further away from the text
%\setlength{\footskip}{90pt}

\renewcommand{\chaptermark}[1]{%
 \markleft{\normalfont\sffamily\thechapter.\ \scshape#1}{}}
\renewcommand{\sectionmark}[1]{%
 \markright{\normalfont\sffamily\thesection.\ #1}{}}
%  \renewcommand{\sectionmark}[1]{%
%  \markboth{\thesection.\ #1 Whatwhat}{}}
% On even pages, put the chapter title into the left header
\lehead{\leftmark}
% On odd pages, put the section title into the right header
\rohead{\normalfont\sffamily\rightmark}
% Clear footer right and left, put page number in center
\lefoot*{}
\rofoot*{}
\cfoot*{\pagemark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Style title page

\date{\CITY, \SUBMISSIONMONTH\ \SUBMISSIONYEAR}
\constructtitle{\vspace{\pretitlewidth}\Huge\TITLE\vspace{\titlesepwidth}}
\ifthenelse{\boolean{dissertation}}{
  % The date should be only the submission year.
  \date{\CITY, \SUBMISSIONYEAR}
  \author{Dissertation zur Erlangung des Grades \\ 
  des Doktors der Naturwissenschaften \\
  der Fakultät für Mathematik und Informatik \\
  der Universität des Saarlandes \\[\authorsepwidth]
  vorgelegt von  \\
  \AUTHOR}
}{
  \date{\CITY, \SUBMISSIONMONTH\ \SUBMISSIONYEAR}
  \author{%
    \Large %
    \UNIVERSITY\\[\medskipamount]
    \DEPARTMENT\\[.9\authorsepwidth]
    \textsc{\THESISKIND's Thesis} \\[.9\authorsepwidth]
    \emph{submitted by} \\
    \AUTHOR\\[.9\authorsepwidth]
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Style the Logo on the Front Page

\ifthenelse{\boolean{logobottom}}{
  \newcommand*\logox{0}
  \newcommand*\logoy{-350}
  \newcommand*\logoopacity{.3}
  \newcommand*\authorsepwidth{2cm}
  \newcommand*\titlesepwidth{1cm}
  \newcommand*\pretitlewidth{0cm}
}{
  \newcommand*\logox{0}
  \newcommand*\logoy{0}
  \newcommand*\logoopacity{.1}
  \newcommand*\authorsepwidth{1cm}
  \newcommand*\titlesepwidth{0cm}
  \newcommand*\pretitlewidth{10cm}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Let figures and tables share counter

\makeatletter
\let\c@table\c@figure{}
\makeatother 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Style ToC and Header

% Set plain page style for ToC/LoF/LoT spanning more than one page.
\AfterTOCHead{\pagestyle{plain}}
\AfterStartingTOC{\clearpage}

% Style ToC/... Header:
% Store the name in old macro to be used in styled version.
\let\oldcontentsname\contentsname{}
\renewcommand{\contentsname}{%
  \huge\sf \rule{\textwidth}{.8pt}\\[\medskipamount]%
  \oldcontentsname\\[-2\medskipamount]
  \huge\sf \rule{\textwidth}{.8pt}
}
\let\oldlistfigurename\listfigurename{}
\renewcommand{\listfigurename}{%
  \huge\sf \rule{\textwidth}{.8pt}\\[\medskipamount]%
  \oldlistfigurename\\[-2\medskipamount]
  \huge\sf \rule{\textwidth}{.8pt}
}
\let\oldlisttablename\listtablename{}
\renewcommand{\listtablename}{%
  \huge\sf \rule{\textwidth}{.8pt}\\[\medskipamount]%
  \oldlisttablename\\[-2\medskipamount]
  \huge\sf \rule{\textwidth}{.8pt}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Background image for title page

% Produce background picture on title page featuring the logo of the university.
\makeatletter
\newcommand{\@printlogo}[1]{
\AddToShipoutPicture*{
    \put(\logox,\logoy){
      \parbox[b][\paperheight]{\paperwidth}{%
        \vfill
        \centering
        \begin{tikzpicture}
          \node [opacity=\logoopacity] (0,0) {
            \includegraphics[%
              height=.8\paperheight,%
              width=.8\paperwidth,%
              keepaspectratio,%
            ]{#1}
          };
        \end{tikzpicture}
        \vfill
      }
    }
  }
}
\newcommand{\printlogotransparentbg}{\@printlogo{logo.png}}
\newcommand{\printlogoopaquebg}{\@printlogo{logo.pdf}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Night Mode Style

\ifthenelse{\boolean{nightmode}}{
  \pagecolor[rgb]{0.2,0.2,0.2}
  \color[rgb]{.9,.9,.9}
  \definecolor{bluekeywords}{RGB}{120, 170, 250}
  \definecolor{greentypes}{RGB}{167, 247, 101}
  \definecolor{redstrings}{RGB}{247, 211, 92}
  \definecolor{graynumbers}{rgb}{0.8, 0.8, 0.8}
  \definecolor{goldcomments}{RGB}{247, 211, 92}
  \renewcommand*\logoopacity{1}
}{
  \definecolor{bluekeywords}{rgb}{0.13, 0.13, 1}
  \definecolor{greentypes}{rgb}{0, 0.5, 0}
  \definecolor{redstrings}{RGB}{171, 114, 2}
  \definecolor{graynumbers}{rgb}{0.5, 0.5, 0.5}
  \definecolor{goldcomments}{rgb}{0.6, 0.4, 0.08}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Theorem Environments

\AtBeginEnvironment{definition}{\Needspace{3\baselineskip}}% \break if fewer than 5\baselineskip is available on page

\declaretheoremstyle[
  headfont=\bfseries,
  numbered=yes, % DONT change, will break everything for some reason.
  bodyfont=\normalfont,
  spaceabove=\topsep,
  postheadspace=1em,
  headpunct={},
  postheadhook=\defheaderline,
  prefoothook=\\*\noindent\defheaderline,
  spacebelow=.5\topsep,  
]{sepdef}

\declaretheorem[
  style=sepdef,
  title=Definition,
  refname={definition,definitions},
  Refname={Definition,Definitions},
  numberwithin=chapter
]{definition}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}{Remark}[section]

\theoremstyle{definition}
\newtheorem{construction}{Construction}[chapter]
% Taken from https://tex.stackexchange.com/a/32394
\newtheorem{examplex}{Example}[section]
\newenvironment{example}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{\(\triangle\)}\examplex}
  {\popQED\endexamplex}
  
  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Table styles

\newcolumntype{L}{>{\(}l<{\)}} % math-mode version of "l" column type
\newcolumntype{R}{>{\(}r<{\)}} % math-mode version of "r" column type
\newcolumntype{C}{>{\(}c<{\)}} % math-mode version of "c" column type

